Liveness Detection Competition -- Noncontact-based Fingerprint Algorithms and Systems (LivDet-2023 Noncontact Fingerprint)

Liveness Detection (LivDet) is an international competition series open to academia and industry with the objec-tive to assess and report state-of-the-art in Presentation Attack Detection (PAD). LivDet-2023 Noncontact Fingerprint is the first edition of the noncontact fingerprint-based PAD competition for algorithms and systems. The competition serves as an important benchmark in noncontact-based fingerprint PAD, offering (a) independent assessment of the state-of-the-art in noncontact-based fingerprint PAD for algorithms and systems, and (b) common evaluation protocol, which includes finger photos of a variety of Presentation Attack Instruments (PAIs) and live fingers to the biometric research community (c) provides standard algorithm and system evaluation protocols, along with the comparative analysis of state-of-the-art algorithms from academia and industry with both old and new android smartphones. The winning algorithm achieved an APCER of 11.35% averaged overall PAIs and a BPCER of 0.62%. The winning system achieved an APCER of 13.0.4%, averaged over all PAIs tested over all the smartphones, and a BPCER of 1.68% over all smartphones tested. Four-finger systems that make individual finger-based PAD decisions were also tested. The dataset used for competition will be available 1 to all researchers as per data share protocol

==> redundant.tex <==
\author{\IEEEauthorblockN{Sandip Purnapatra}
\IEEEauthorblockA{\textit{ECE Department} \\
\textit{Clarkson University}\\
Potsdam, USA \\
purnaps@clarkson.edu}
\and
\IEEEauthorblockN{Humaira Rezaie}
\IEEEauthorblockA{\textit{CS Department} \\
\textit{Clarkson University}\\
Potsdam, USA \\
rezaieh@clarkson.edu}
\and
\IEEEauthorblockN{Bhavin Jawade}
\IEEEauthorblockA{\textit{CS Department} \\
\textit{University at Buffalo}\\
Buffalo, NY, USA \\
bhavinja@buffalo.edu}
\and
\IEEEauthorblockN{Yu Liu}
\IEEEauthorblockA{\textit{CS Department} \\
\textit{Clarkson University}\\
Potsdam, USA \\
liuy5@clarkson.edu}
\and
\IEEEauthorblockN{Yue Pan}
\IEEEauthorblockA{\textit{CS Department} \\
\textit{Clarkson University}\\
Potsdam, USA \\
yuepan@clarkson.edu}
\linebreakand
\IEEEauthorblockN{Luke Brosell}
\IEEEauthorblockA{\textit{ECE Department} \\
\textit{Clarkson University}\\
Potsdam, USA \\
brosellr@clarkson.edu}
\and
\IEEEauthorblockN{Mst Rumana Sumi}
\IEEEauthorblockA{\textit{ME Department} \\
\textit{Clarkson University}\\
Potsdam, USA \\
sumima@clarkson.edu}
\and
\IEEEauthorblockN{Lambert Igene}
\IEEEauthorblockA{\textit{ECE Department} \\
\textit{Clarkson University}\\
Potsdam, USA \\
igenela@clarkson.edu}
\and
\IEEEauthorblockN{Alden Dimarco}
\IEEEauthorblockA{\textit{HSE Program} \\
\textit{Clarkson School}\\
Potsdam, USA \\
dimarc@clarkson.edu}
\and
\IEEEauthorblockN{Srirangaraj Setlur}
\IEEEauthorblockA{\textit{CS Department} \\
\textit{University at Buffalo}\\
Buffalo, NY, USA \\
setlur@buffalo.edu}
\linebreakand
\IEEEauthorblockN{Soumyabrata Dey}
\IEEEauthorblockA{\textit{CS Department} \\
\textit{Clarkson University}\\
Potsdam, USA \\
sdey@clarkson.edu}
\and
\IEEEauthorblockN{Stephanie Schuckers}
\IEEEauthorblockA{\textit{ECE Department} \\
\textit{Clarkson University}\\
Potsdam, USA \\
sschucke@clarkson.edu}
}
\IEEEoverridecommandlockouts
\IEEEpubid{\makebox[\columnwidth]{979-8-3503-3607-8/23/\$31.00 ~\copyright2023 IEEE \hfill}}
\hspace{\columnsep}\makebox[\columnwidth]{ }}


\section{Noncontact Fingerprint PAD efforts so far}
Many researchers have been exploring smartphone-based finger photo recognition in the last decades \cite{lee2006preprocessing} \cite{lee2008recognizable} \cite{li2012testing} \cite{sankaran2015smartphone} \cite{jawade2021multi} \cite{jawade2022ridgebase}. Most of these works were focused on finger photo-processing techniques i.e. segmentation, enhancement for finger photo quality improvements, and conversion from finger photos to digital fingerprints. These converted digital fingerprints were then used minutia-based matching algorithms to demonstrate improvement in authentication performances. These researches demonstrated the challenges of finger photo processing, however, the corresponding dataset were not made available publicly to encourage further research. Early in the last decade, Stein et al. \cite{stein2013video} developed a PAD algorithm for PAI detection in a smartphone-based noncontact fingerprint-capturing application. The algorithm used the reflection properties of the PAIs as hand-crafted features and analyzed the frames of a finger video. The authors achieved a 77\% successful detection rate, however, assumed the PAIs i.e. finger photo printouts or finger sleeves would have different reflection properties than live fingers without elaborating more about the assumption. Additionally, it is not clear from the results if finger sleeves laid on top of live fingers would be accurately detected using this method. Another work from the authors of Taneja et al. \cite{taneja2016fingerphoto} studied finger photo PAD on mobile devices with print-out and replay attacks. The authors successfully classified between the live and PAI samples using a Support Vector Machine (SVM) algorithm with hand-crafted texture-based features and achieved a detection equal error rate (D-EER) of 3.71\%. The PAD dataset is publicly available, however, the manual capture of live and finger photos was not properly focused and thus of low quality and noisy, and neither data was collected using standard international collection protocols. Fujio et al. \cite{fujio2018face} used the same dataset and developed a PAD algorithm based on CNN (AlexNet) architecture. The algorithm detected the noise of the PAI images and achieved a half-total error rate of 0.04\%. Interestingly, the authors resized the training images to 256*256 dimensions for analysis. Resizing or down-sampling images raises the chance of loss of further features in the unfocused dataset and might not provide a good classification against high-quality PAIs. The same PAD dataset, along with collected replay attack data, was used by the authors Marasco et al. \cite{marasco2021fingerphoto} to achieve D-EER of 2.14\% with AlexNet and 0.97\% with ResNet. The authors evaluated different color spaces and CNN architectures, however, the publication did not mention any details or report on the image quality issues in the publication. Wasnik et al. \cite{wasnik2018presentation} published PAD-based finger photo recognition. The authors converted the finger photos and replay attacks to traditional digital fingerprints and derived hand-crafted features like second-order local structures and classified between the live and PAI images using an SVM algorithm to achieve 4.43\% D-EER. \par 

Recently, Kolberg et al. \cite{kolberg2023colfispoof} introduced the {\bf COLFISPOOF} dataset for non-contact fingerprint PAD. The dataset has 7200 samples of 72 different PAI species and was captured using two different smartphones. We applaud their effort to collect such large-scale data for deep neural network-based training. \iffalse However, the dataset was created using only 8 different PAI materials i.e. knetosil, mould glue, latex, silly putty, paper prints (grey-scale and RGB), school glue, and dragon skin.\fi Most notably, the PAI materials used by the authors are mostly silicon-based and of FIDO level A \& B difficulty, which translates to easy and moderately difficult to make. Furthermore, the authors used {\bf SynCoLFinGer} \cite{priesnitz2022syncolfinger}, which synthetically simulates and generates finger photos from contact-based fingerprints. These synthetic live fingerprints can be very easily visually distinguished from the live fingertips. The authors also proposed evaluation protocols to train and test the PAD algorithms using the developed dataset but did not contribute any PAD algorithm.  \par
\iffalse
\begin{figure}[htbp]
\centerline{\includegraphics[height=5cm,width=0.4\textwidth]{Images/simulated_noncontact.png}}
\caption{Live Finger photo Vs. SynCoLFinger photo}
\label{SynCol}
\end{figure}
\fi
From the evaluation of the state-of-the-art, evidently, the studies that have shared data sets publicly do not have a large spectrum of PAIs, made in accordance with FIDO or ISO standards. The datasets that can be found in the public domain are of low quality, not in focus. Most PAIs have only used finger sleeves or PAIs made artificially from different materials to lay on fingertips to obscure real fingertips, finger photos printouts, and display attacks as PAIs. None of the studies used extremely sophisticated, hard-to-make, and visually indistinguishable synthetic PAIs to test their developed algorithms. Neither the algorithms were tested against unseen or unknown PAI varieties to replicate real-life uncertain scenarios. Our previous work \cite{purnapatra2023presentation} developed a PAD dataset according to the standard PAI creation protocols, and of three different difficulty levels, using different types of materials and PAI textures that reflect real skin tones. This work also contributed deep neural network-based architectures like DenseNet-121 and NASNetMobile for presentation attack detection using the developed dataset. The DenseNet-121 model achieved APCER$_{\mbox{\footnotesize average}}$ of 0.07\% against known PAIs, a 21.08\% against all PAIs, and BPCER of 0.18\%. While the DenseNet-121 Keras version of the model achieved APCER$_{\mbox{\footnotesize average}}$ of 13.74\% against all PAIs. Although the dataset used was still under development, and there was scope for further improvement in the performance of our models, we realized the absence of any standard comparison of models and their results across academia and industry. Thus, we decided to host the LivDet-2023 Noncontact Fingerprint Algorithms and Systems competition and invited participants across the industry and academia to participate and compare performances. 
We used the \cite{purnapatra2023presentation} publication dataset and further enhanced the number of samples by finishing the PAI collection. To ensure capture quality the capture process was manual and arduous, however, it was finished just in time for the competition. So, all the PAI images used in the LivDet-2023 Noncontact fingerprint Algorithms competition were collected manually by focusing on the target fingertip and quality was checked to ensure the fingertip is in focus and of good quality i.e. not blurred or smudged and fingertip ridges and valleys are clearly visible.
